Only YOU Can Make IEEE VIS Environmentally Sustainable

The IEEE VIS Conference (or VIS) hosts more than 1000 people annually. It brings together visualization researchers and practitioners from across the world to share new research and knowledge. Behind the scenes, a team of volunteers puts together the entire conference and makes sure it runs smoothly. Organizing involves logistics of the conference, ensuring that the attendees have an enjoyable time, allocating rooms to multiple concurrent tracks, and keeping the conference within budget. In recent years, the COVID-19 pandemic has abruptly disrupted plans, forcing organizers to switch to virtual, hybrid, and satellite formats. These alternatives offer many benefits: fewer costs (e.g., travel, venue, institutional), greater accessibility (who can physically travel, who can get visas, who can get child care), and a lower carbon footprint (as people do not need to fly to attend). As many conferences begin to revert to the pre-pandemic status quo of primarily in-person conferences, we suggest that it is an opportune moment to reflect on the benefits and drawbacks of lower-carbon conference formats. To learn more about the logistics of conference organizing, we talked to 6 senior executive-level VIS organizers. We review some of the many considerations that go into planning, particularly with regard to how they influence decisions about alternative formats. We aim to start a discussion about the sustainability of VIS -- including sustainability for finance, volunteers, and, central to this work, the environment -- for the next three years and the next three hundred years.

==> preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etal}
{et al.}
%% {et al.\@ }
\newcommand{\etals}
{et al.'s}
%% {et al.\@'s }  

\newcommand{\ie}{{i.e.,}}
\newcommand{\eg}{{e.g.,}}
\newcommand{\etc}{{etc.}}
\newcommand{\cf}{{cf.}}
\newcommand{\ala}{\`a la}
\newcommand{\toolName}[1]
%% {\textsc{#1}}
{#1}

\newcommand\elr[1]{{\color{teal}[ELR: #1]}}
\newcommand\am[1]{{\color{orange}[AM: #1]}}

\newcommand{\figref}[1]{\hyperref[#1]{Fig.~\ref*{#1}}}
\newcommand{\secref}[1]{\hyperref[#1]{Sec.~\ref*{#1}}}


\newcommand{\footnoteWithIndent}[1]
%% {\footnote{\mbox{}{#1}}}
{\footnote{#1}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% \def\parahead#1
%%   %% {\paragraph{\textbf{#1.}}}
%%   {\paragraph{\textit{#1.}}}

\newcommand{\parahead}[1]
{%
  \paraheadd{#1}.
}

\newcommand{\paraheadd}[1]
{%
  \vspace{0.07in}%
  \noindent%
  \textbf{\textit{#1}}%
}

% \def\subsubsec#1
%   {\subsubsection*{\textit{#1}}}

\def\subsubsec#1
{\subsubsection{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\inlineFig}[1]{%
  \begingroup\normalfont
  % \vspace*{-0.1cm}
  \includegraphics[height=1.2\fontcharht\font`\B]{#1}%
  \endgroup
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\hlc}[2][yellow]{{%
                  \colorlet{foo}{#1}%
                  \sethlcolor{foo}\hl{#2}}%
}
\newcommand\qt[1]{\hlc[SeaGreen!15]{``#1''}}
\newcommand{\pxx}[1]{\textbf{P$_{#1}$}}

\usepackage[normalem]{ulem}
\definecolor{linkColor}{HTML}{257E98}
\setuldepth{Berlin}
\newcommand\asLink[2]{\textcolor{linkColor}{\href{#1}{\ul{#2}}}}


\newcommand{\osf}{\asLink{https://osf.io/u2eps/}{osf.io/u2eps/}}
